Inter-Domain Routing with Extensible Criteria

With the rapid evolution and diversification of Internet applications, their communication-quality criteria are continuously evolving. To globally optimize communication quality, the Internet's control plane thus needs to optimize inter-domain paths on diverse criteria, and should provide flexibility for adding new criteria or modifying existing ones. However, existing inter-domain routing protocols and proposals satisfy these requirements at best to a limited degree. We propose IREC, an inter-domain routing architecture that enables multi-criteria path optimization with extensible criteria through parallel execution and real-time addition of independent routing algorithms, together with the possibility for end domains to express their desired criteria to the control plane. We show IREC's viability by implementing it on a global testbed, and use simulations on a realistic Internet topology to demonstrate IREC's potential for path optimization in real-world deployments.

==> analysis.tex <==

\section{Analysis} \label{sec:analysis}
In this section, we analyze \system{}'s scalability and security.


\subsection{Scalability}
In contrast to data plane operations, control plane operations are not particularly performance-critical.
Still, \system{} minimizes communication between different entities and provides AS operators with configuration options that allow distributing \system{}'s state and computation overhead among multiple (physical or virtual) appliances.

\paragraph{Communication}

\begin{itemize}
    \item  Duplicate PCBs are filtered\\
    \item \todo{Compute upper bound of sent PCBs, storage overhead etc.?}
    \item On an abstract level, it is sufficient that each RAC from one AS only sends routing messages to RACs of neighboring ASes with the same routing algorithm.
    \item However, this requires the negotiation of neighboring ASes, and may cause lots of repetitive routing messages, as different algorithms may disseminate the same paths.
    \item PCBs are first sent to the ingress gatway (instead of every RAC sending to its corresponing RAC in the neighboring AS) -> less inter-domain communication overhead
    \item Egress gateway filters duplicate paths.
    \item Number of PCBs would be tremendously high if every RAC would itself add only the information it needs to each PCB (and then sign it).
    \item RACs inside an AS are independent, i.e., they do not need to communicate with each other.
\end{itemize}

\paragraph{Computation and Storage}
\begin{itemize}
    \item Describe which components can be run on separate machines. (RACs, databases, one Ingress Gateway and one Egress Gateway per interface etc.)
    \item Ingress database can be done per ingress interface, an be further split up into databases for different source ASes.
\end{itemize}

\subsection{Security}

\begin{itemize}
    \item Possible attacks and their mitigation (mainly due to putting algorithms in routing messages)
    \item Algorithms/boxes implementations should be flexible to prevent one potentially malicious entity to distribute their version of an algorithm.
    If an AS uses only / mostly algorithms issued by this entity, this is problematic: the algorithms could be defined to only allow paths through certain ASes, basically resulting in a hijacking attack.
    A possible solution could be to require open source algorithms, or to just specify the algorithm/box definition as pseudo code.
    \item We can use certificates to authenticate the RACs towards the ingress and egress gateways.
    \item An AS can potentially do hijacking by promoting perfect metadata.
    \item It even becomes simpler to do coremelt/crossfire attacks? (Though this is probably already possible in SCION as of now)
\end{itemize}



==> bootstrapping_connectivity.tex <==

\todo{For the ICNP submission, no appendix is allowed.}

\subsection{Bootstrapping Connectivity}
ASes that are disconnected from other ASes over a long time period, as well as newly joining ASes, should be able to quickly (re-)establish connectivity.
In particular, this includes (i) finding paths to other ASes and (ii) disseminating self-originated PCBs throughout the Internet.
\system{} provides mechanisms to achieve this in the order of a \textit{single round trip}.

First, for getting paths to other ASes, the ingress gateway of the AS that needs to bootstrap connectivity can request PCBs from the egress gateways of its neighboring ASes.
In case the neighboring ASes also do not have any paths available, the process continues recursively.

Second, to achieve rapid PCB dissemination from the AS that has recently joined the network, a dedicated static RAC uses the subscription and notification mechanism provided by the ingress gateway.
The RAC gets notified about new PCBs immediately, and forwards them directly to the egress gateway.
To ensure the scalability of this approach, the RAC only guarantees each origin AS to forward a single (potentially sub-optimal) PCB per certain time interval.
Therefore, already the first PCB sent by an AS (re-)connecting to the Internet is propagated immediately through the whole network.

\todo{Explain subscription and notification mechanism.}

\todo{At the moment, the egress gateway only stores the hash of the PCBs. With this proposal, the egress gateway needs to keep a database with at least one current PCB per origin AS.}


% RACs can additionally subscribe at the ingress gateway to get notifications about incoming PCBs with path metadata matching their criteria.
% Example notification: there is a new PCB originating from AS X. (There criteria here would be simply the source AS.)
% The RAC still needs to pull the actual PCBs ifself, it is not contained in the notification.
%



% \todo{Limited number of paths, e.g., to core ASes}

% \todo{(Note that this is not the same as in "Immediate PCB Propagation".}

% Only works if neighbor supports our system.

==> introduction_old.tex <==
\section{Introduction}\label{sec:intro}

\begin{sloppypar}
Operators of large wide-area networks~(WANs) have long realized the importance of \emph{intra-domain} path optimization based on demand and traffic characteristics. 
In these networks, often based on software-defined networking (SDN), centralized controllers (i) monitor the state of the network and analyze the specific requirements of traffic flows; (ii) optimize the network paths and assign them to flows according to such requirements; and (iii) constantly and rapidly update to accommodate new applications with different path-optimization criteria~\cite{Jain:2013:B4, Yap:2017:espresso}. These networks thus provide a flexible and performant platform, where traditional applications thrive and new ones can evolve, such as cloud-based gaming~\cite{forbes-online-gaming} or holographic communication~\cite{Ha:2022:holographic}.

% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% marc.wyss: Why those examples?
% It seems they just need low latency and high throughput.
% G-SINC (attack-resisilient time sync) relying on disjoint paths could be a more interesting example?
% May 15, 2023 11:17 AM
% tabaeeali: Can you add it Marc?
% May 24, 2023 10:52 AM
% marc.wyss: Done
% May 27, 2023 7:51 AM
% tabaeeali: But now that we do not say it requires disjointness, it feels odd.
% May 27, 2023 1:11 PM
% tabaeeali: I mean other applications are pretty known, but nobody knows G-SINC
% May 27, 2023 1:11 PM

% option 2
%---Byzantine fault-tolerant clock synchronization and holographic communication are recent examples~\cite{G-SINC,Ha:2022:holographic}---can evolve.
%
In contrast, the scale and complexity of \emph{inter-domain} routing has prevented analogous advancements on the Internet to this point.
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% tabaeeali: Adrian's suggestion here: "In contrast, the ossification of inter-domain routing, has prevented the evolution of BGP."
% May 29, 2023 6:30 PM
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% tabaeeali: Adrian said: "analogous to what? the evolution of existing algorithms?"
% May 29, 2023 7:11 PM

Today, Internet path optimization is limited to coarse-grained strategies, such as selective prefix announcements~\cite{Cardona:2016:bgp_filtering} and BGP communities~\cite{Borkenhagen:2019:bgp_communities}; only the largest Internet service providers (ISPs) and content-distribution networks (CDNs) can afford to deploy anycast routing to boost last-mile performance.

Path-aware networks (PANs) emerged as a new paradigm to introduce more granular inter-domain path optimization.
PAN architectures~\cite{Segment_Routing, Chuat2022SCION,Pathlets} expose multiple paths to applications at the endpoints, allowing them to select the best path based on application requirements. 
They also provide endpoints with performance metrics such as latency and bandwidth in routing messages, informing endpoints' decision.
While requirement-aware path selection at the endpoints can significantly improve the communication quality compared to today's single-path Internet~\cite{conext2021deployment}, it still cannot compete with the optimization granularity of intra-domain networks. 
%
---Unlike controllers in a centralized WAN, 
autonomous systems (ASes) do not have full visibility on the inter-domain topology, and they are oblivious to the requirements of endpoints outside their domains. 
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% tabaeeali: Adrian wants the to be removed. But ASes are not oblivious to the requirement of endpoints in their own domain.
% May 29, 2023 7:23 PM
Furthermore, the distributed nature of inter-domain routing requires standardization and vendor support, significantly slowing down updates to the routing infrastructure~\cite{Wirtgen:2023:xbgp}, thus, limiting extensibility and hindering innovation.
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% tabaeeali: Adrian syas: "ossification"
% May 29, 2023 7:14 PM

In this work, we enable evolution in inter-domain routing by introducing \system{}, a control-plane architecture for PANs that (i)  achieves multi-criteria inter-domain path optimization, and (ii) allows \emph{criteria extensibility}. We define criteria extensibility as the ability to modify path optimization criteria according to application or network requirements without interrupting connectivity or disrupting control-plane functionality and with low effort, i.e., requiring no standardization or vendor implementation, and minimal deployment effort by network operators. To satisfy these objectives, \system{} takes advantage of the ability of PAN architectures to scalably discover and use additional paths without disrupting the use of already discovered paths enabled by the clear separation of data and control planes in such architectures. 

Building on these properties, \system{} introduces the concept of independent path optimization on separate sets of application-wise criteria by parallel execution of multiple routing algorithms (\Cref{sec:principles:parallel}). Each AS has the choice of which algorithms to deploy, and new algorithms can be dynamically loaded into the system without compromising other live routing processes. The core challenges are to ensure the scalability of the system with regard to the number of parallel routing algorithms and the consensus among ASes to optimize paths according to the same criteria to prevent routing inconsistency, yet ensuring extensibility. To address these challenges, we introduce the concept of \emph{on-demand routing} 
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% marc.wyss: Not sure it is critical, but the term on-demand routing seems to be already widely used: https://en.wikipedia.org/wiki/On_Demand_Routing
% May 15, 2023 2:25 PM
(\Cref{sec:principles:on_demand}), whereby end domains express their optimization criteria for paths ending at them by communicating routing algorithms via routing messages. New routing algorithms can therefore be deployed in real time, without touching the existing infrastructure. 
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
% tabaeeali: Adrian says "extending". But, this is not what touching means here. It means effortless.
% May 29, 2023 6:07 PM
% marc.wyss: changing / modifying maybe?
% May 30, 2023 11:10 AM
Finally, we also design a \emph{pull-based routing} mechanism (\Cref{sec:principles:pull_based}), that allows traffic \emph{sources} to request paths with specific characteristics towards a destination---the opposite of traditional \emph{destination}-generated routing messages.
\todo{@giacomo: talk about standardization}
\todo{@giacomo: talk a bit about how the layers communicate with each other, and we find basic paths (backward compatibility with legacy SCION)}

% 

Our implementation demonstrates \system{}'s practical viability, and our simulations show 
% its scalability to Internet-scale topologies and 
its potentials for optimizing on multiple criteria in an Internet-scale topology.

\paragraph{Contributions} In summary, we contribute towards a performant and fast-evolving Internet as follows:
\begin{itemize}
    \item Designing \system{}, enabling multi-criteria inter-domain path optimization with extensible criteria through (i) parallel routing algorithms(\Cref{sec:principles:parallel}), (ii) on-demand routing (\Cref{sec:principles:on_demand}), and (iii) pull-based routing (\Cref{sec:principles:pull_based}).
    \item Suggesting a standardization model 
    % ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW;
%     tabaeeali: not clear for Adrian.
% May 29, 2023 6:57 PM
% marc.wyss: This can be shortened after Giacomos changes to the introduction.
% May 30, 2023 7:33 PM
    for \system{}'s features, to reconcile extensibility with safe deployment in an open and distributed Internet, without a centralized controller, and without causing routing inconsistencies (\Cref{sec:deployment_standardization}), 
    \item Implementing \system{} in the open-source codebase~\cite{scionproto} of a PAN architecture, SCION~\cite{Chuat2022SCION}, and evaluating its performance, (\Cref{sec:implementation}),
    \item Evaluating \system{} on a realistic Internet topology using an ns-3~\cite{nsnam_ns-3_nodate} based simulator~\cite{scion-sim}, showing its optimization potentials on multiple criteria (\Cref{sec:simulations}).
\end{itemize}



\end{sloppypar}





















 



==> makefile <==
FILES = paper
# FILES = $(patsubst %.tex,%,$(wildcard *.tex))
FILES_PDF = $(addsuffix .pdf,$(FILES))
FILES_FINAL_PDF = $(addsuffix -final.pdf,$(FILES))
FILES_DIFF_PDF = $(addsuffix -diff.pdf,$(FILES))

# specifies which revision to create the diff against
rev=prerevision

# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
.PHONY: $(FILES_PDF) $(FILES_FINAL_PDF) $(FILES_DIFF_PDF) all clean final diff.pdf final-submission.tar.gz

# The first rule in a Makefile is the one executed by default ("make"). It
# should always be the "all" rule, so that "make" and "make all" are identical.
all: $(FILES_PDF) $(FILES_FINAL_PDF)

final: $(FILES_FINAL_PDF)

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

#%.tex: %.raw
#        ./raw2tex $< > $@

#%.tex: %.dat
#        ./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

final-submission.tar.gz:
	rm -rf final-submission
	rm -f final-submission.tar.gz
	mkdir final-submission/ && mkdir final-submission/figures && cp paper.tex acmart.cls ACM-Reference-Format.* references.bib rfc.bib abstract.tex intro.tex background.tex deployment.tex beaconing.tex eval.tex related.tex algorithm.tex final-submission/ && cp figures/isp.pdf figures/enddomain5.pdf figures/ixp.pdf figures/pathdump_max_link_failures-detail-comparison-p100.pdf figures/pathdump_max-capacity-in-link-units.pdf figures/SCIONLab_overhead.pdf figures/cost_cdf.pdf figures/2000_geo_rel_max_link_failures-detail-comparison-15.pdf figures/2000_geo_rel_max-capacity-in-link-units.pdf figures/beaconing_v4.pdf final-submission/figures
	tar -czvf $@ final-submission/

$(FILES_PDF): %.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape $<

$(FILES_FINAL_PDF): %-final.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\newcommand{\final}{}\input{%S}"' $<

%-diff.tex: %.tex
	$(eval old_revision_dir := $(shell mktemp -d))
	git worktree add "$(old_revision_dir)"
	cd "$(old_revision_dir)" && git checkout "$(rev)"
	latexdiff --flatten $(old_revision_dir)/$< $< >$@
	git worktree remove "$(old_revision_dir)"
	$(RM) -rf "$(old_revision_dir)"

$(FILES_DIFF_PDF): %-diff.pdf: %-diff.tex
	latexmk -pdf -use-make $<
	$(RM) $<

clean:
	latexmk -c
	$(RM) *.log
	$(RM) -r *.prv
	$(RM) *.bbl
	$(RM) *-diff.tex
	$(RM) *.synctex.gz
	$(RM) *.fdb_latexmk
	$(RM) *.fls
	$(RM) *.aux
	$(RM) *.blg
	$(RM) *.out


==> problem_statement_old.tex <==

\section{Problem Statement}\label{sec:statement}

\subsection{Motivation}\label{sec:statement:motivation}
\paragraph{Multi-Criteria Path Optimization}\label{sec:statement:motivation:multi_criteria} Network endpoints typically have application-specific communication-quality criteria, for which the control plane should ideally provide optimal paths. However, in the scope of inter-domain routing, despite the diversity of potentially discoverable paths~\cite{conext2021deployment}, paths are usually optimized on a few static criteria such as AS-hop length while respecting business relationships.

\paragraph{Criteria Extensibility}\label{sec:statement:motivation:extensibility} As applications continue to evolve, so do their communication requirements. Additionally, ASes need to continuously adjust their routing decisions as the result of network changes, or routing policy updates. Optimizing paths on extensible criteria is thus the ability to modify path optimization criteria according to application or network requirements without interrupting connectivity or disrupting control-plane functionality and with low effort, i.e., requiring no standardization or vendor implementation, and minimal deployment effort by network operators.
% needs an extensible control plane that allows the low-effort adjustment of routing criteria and the introduction of new ones. 
However, in current inter-domain routing, such adjustments require standardization efforts, which often unfold over a period of a decade~\cite{Wirtgen:2023:xbgp}, and then require implementation by vendors, and finally deployment by network operators. 
% This significant delay impedes the control plane from adapting to the requirements of emerging applications and hinders innovation. 
How to shorten decades-long innovation cycles in inter-domain routing and enable support for emerging application requirements is an intriguing research challenge.
The significance of the problem is well underscored by the multitude of research studies, such as XIA~\cite{Naylor:2014:XIA}, Trotsky~\cite{McCauley2019Trotsky}, and xBGP~\cite{Wirtgen:2023:xbgp}, which take significant steps in making  inter-domain routing extensible. 
\subsection{Terminology}\label{sec:motivation:terminology}


An \emph{optimality criterion} $C$ describes a relative preference among \emph{attributes} and can be modeled as a total order $\preceq_C$ on them~\cite{Sobrinho:2020:multiple_optimality}. Every path has one attribute $a$, which is a tuple of the values of different \emph{performance metric}s associated with the path. For example, $(w_1, l_1)$ could be the attribute of path $p_1$, where $w_1$ and $l_1$ are  values for the capacity and latency metrics, respectively. Each criterion takes into account a non-empty subset of possible performance metrics $M$. 

We define \emph{multi-criteria path optimization} as path discovery between every pair of ASes $\{s, t\}$ in the network  such that the set of discovered paths contains paths ranked the highest by every total order $\preceq_C$ for every criterion $C$ desired by endpoints and applications in $s$ or $t$ for reaching the other AS.
We define \emph{criteria extensibility} as the ability to add any new criterion to and remove any existing criterion from the criteria on which the control plane is optimizing paths, with low effort, i.e., no standardization or vendor implementation requirement and minimal changes to the existing system, and without affecting optimality on other criteria, or causing instability in the network.


% 



\subsection{Desired Properties}\label{sec:statement:properties}
To realize our objectives, we seek the following properties in a control-plane design: 
\begin{itemize}
    \item[\textbf{P1}] Ability to find optimal paths on multiple criteria.
    \label{p1}
    \item[\textbf{P2}] Independent selection of criteria by each AS.\label{p2}
    \item[\textbf{P3}] Real-time, low-effort, and interruption-free addition and removal of criteria.\label{p3}
    \item[\textbf{P4}] Ability to optimize paths on the criteria of both source and destination ASes of data packets.\label{p4}
    \item[\textbf{P5}] Providing means of optimality guarantee for any criterion.\label{p5}

\end{itemize}



\subsection{Existing Methods and Limitations}\label{sec:statement:existing_methods}

\paragraph{Multi-Criteria Path Optimization} Existing methods jointly optimize paths on all criteria existing in the whole network using a single logic either by defining a single total order on all criteria and optimizing on that total order, or by defining a partial order on the intersection of all criteria and selecting the set of dominant paths, i.e., the ones to which no other path is preferable and which are incomparable among each other.

A multi-criteria total order cannot guarantee optimality because total orders on real-world attributes are not usually isotone on the path extension operation\footnote{Two attributes are isotone for path extension if their relative preference is preserved when both are extended by the same third attribute.}~\cite{Sobrinho:2020:multiple_optimality} while vectoring protocols like BGP need isotonicity to guarantee optimality~\cite{Gouda:2003:Maximizable,Sobrinho:2002:algebra,Sobrinho:2019:fundamental}. This problem is aggravated by the increasing number of considered criteria. Although, dominant attributes on partial orders can guarantee optimality, the number of incomparable paths significantly increases by multiplying the number of criteria in the intersection, resulting in significant communication cost. Furthermore, both methods hinder extensibility as they (i) complicate the optimization logic, (ii) require all ASes to deploy the same logic, and (iii) require interruption and modification of already-existing optimization logic to add any new criterion.

\paragraph{Extensibility}
Both Trotsky~\cite{McCauley2019Trotsky} and xBGP~\cite{Wirtgen:2023:xbgp} takes significant steps towards a highly extensible Internet. Trotsky enables the introduction of new designs and Internet architectures through its backward-compatible framework, and xBGP enables BGP to extend through user-defined eBPF bytecodes. However, none of them consider multi-criteria path optimization as a design objective.
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW  %
% giac.giuliari: maybe add a sentence explaining why these methods fail to achieve the goal? Or point to related work? May 23, 2023 6:17 PM %



\subsection{Challenges}\label{sec:statement:challenges}

\paragraph{Scalability}\label{sec:statement:challenges:scalability}
Different network paths may be optimal for different criteria. Thus, finding optimal paths on all criteria requires multipath routing and forwarding. In stateful multipath proposals, the routing and forwarding state at a router grows linearly with the number of paths. Therefore, the limited forwarding and routing memory in routers impedes scalability regarding number of paths, and in turn, the scalability regarding number of optimization criteria. Furthermore, required computational resources for optimizing paths on multiple criteria can limit scalability to large number of criteria. 

\paragraph{Forwarding Stability} Multi-criteria path optimization can  destabilize stateful forwarding by: (i) increasing routing convergence time for discovering multiple paths, and (ii) increasing the probability of path changes on routers because of the increased probability of change in any of multiple performance metrics compared to a single performance metric. 
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW ;
% giac.giuliari: This is a bit naive. We solve all these challenges by basically having multiple disjoint control planes in parallel.
% May 23, 2023 6:34 PM
% marc.wyss: Can you elaborate a bit more on that? (Or have a suggestion how to solve it?)
% May 24, 2023 4:46 PM

% SECOND COMMENT;
% marc.wyss: can this be simplified?
% May 26, 2023 8:47 AM
Both can lead to transient forwarding loops and blackholes, and thus, disconnectivity. Extensibility can also cause instability in stateful forwarding: modifying routing decisions can change preferred paths, thus, can cause transient loops and blackholes.


\paragraph{Optimality vs. Extensibility}
To guarantee connectivity and optimality on any criterion, all ASes need to agree on (i) optimizing that criterion, and (ii) the format of routing messages. Such requirements impede extensibility, as it needs significant effort to ensure all ASes optimize on the same criteria. Therefore, the main challenge is to reconcile extensibility with optimality and connectivity guarantee.
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW: marc.wyss: guarantees?
% May 30, 2023 11:18 AM


% \paragraph{Routing Consistency} 
% To guarantee path optimization on a criterion, all ASes need to agree on optimizing that criterion. Furthermore, the disagreement of ASes over the format of routing messages can prevent them from communicating and discovering paths, resulting in disconnectivity, or from correctly interpreting path attributes, resulting in sub-optimal paths. Such requirements impede extensibility, as it needs significant effort to ensure all ASes optimize on the same criteria. The main challenge is to reconcile extensibility with optimality guarantee.
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW: 
% giac.giuliari: This is an important and interesting point, I would expand on it a bit more / give it more prominence.
% May 23, 2023 6:28 PM
% tabaeeali: how would you extend on that?
% May 24, 2023 5:20 PM
% 

\paragraph{Usability}
The ultimate goal of multi-criteria path optimization is to satisfy traffic flows' requirements. This requires the \emph{data plane} to be also aware of these requirements and forward each traffic flow on the most suitable path(s). 
However, such a mechanism is currently missing in the inter-domain data plane. 
% ORIGINALLY THERE WAS A COMMENT HERE, BUT REMOVED FOR OVERVIEW: 
% marc.wyss: in tSSSSSSSSShe current Internet?
% May 30, 2023 11:19 AM
For this reason, we build \system{} within the scope of a path-aware network architecture.



==> standardization_deployment.tex <==

\section{Standardization and Deployment}\label{sec:deployment_standardization}
In this section, we propose standardization efforts and deployment requirements necessary to achieve optimality (\hyperref[p5]{P5}) while ensuring ASes can freely choose routing algorithms (\hyperref[p2]{P2}) and new algorithms can be added in real-time (\hyperref[p3]{P3}).


\subsection{Motivation}\label{sec:deployment_standardization:motivation}
A fundamental requirement of distributed routing protocols to accomplish their tasks is that all participating nodes run the same algorithm and use the same routing message format. This has motivated the large body of routing protocol standards both in intra- and inter-domain routing. \system{} is no exception: guaranteeing connectivity and optimality of paths on each set of criteria requires standardization of algorithms and their deployment by all ASes.

However, theses requirements impede extensibility as they contradict the free choice of algorithms by ASes (\hyperref[p2]{P2}), and the lengthy process of standardization (\Cref{sec:statement:motivation:extensibility}) is in contradiction with effortless addition of new algorithms (\hyperref[p3]{P3}). Therefore, we need an effective method for reconciling extensibility with standardization and deployment requirements.

\subsection{Criticality-Oriented Standardization and Deployment}\label{sec:deployment_standardization:criticality}

Not all control plane tasks are of the same criticality for the network, meaning that, the answer to ``how severely would it impact the network if a task is not fully accomplished'' differs for different tasks. For instance, more fundamental tasks, e.g., providing connectivity, have higher criticality as its partial accomplishment can cause disconnectivity in the Internet.

We leverage this difference in the criticality of control-plane tasks to reconcile extensibility with standardization and deployment requirement by proposing the following standardization and deployment paradigm. More critical tasks require more standardization efforts and stricter deployment requirements to ensure their accomplishment while less critical tasks need less standardization efforts and looser deployment requirements to enable extensibility. What facilitates such a paradigm in \system{} is its parallel routing algorithm mechanism (\Cref{sec:principles:parallel}), which allows tasks of different criticality to run in parallel without interrupting and affecting each other.

\subsection{Tiers of Criticality}\label{sec:deployment_standardization:tiers_criticality}

We identify three tiers of criticality for different control-plane tasks: (i) \emph{highly critical}, i.e., guaranteeing global connectivity by discovering at least one path between any pair of ASes, where failure to accomplish has the detrimental consequence of cutting some parts of the Internet from the rest, (ii) \emph{moderately critical}, i.e., optimizing paths on basic criteria, such as low latency, where failure to accomplish can interrupt many applications or deteriorates their communication quality, (iii) \emph{non-critical}, i.e., optimizing paths for arbitrary criteria of specific applications, where failure to accomplish only impacts the communication quality of those applications.

Based on these three criticality tiers, we propose different levels of standardization efforts and deployment requirements for different algorithms. Furthermore, we identify efforts and requirements that are specific to functionality of \system{}, but not algorithms.

\subsection{Standardization Effort}\label{sec:deployment_standardization:standardization}
% We define one standardization tier per criticality tier. In each tier, we specify standardization requirements for (i) algorithms, (ii) their implementation, and (iii) PCB format.
 
\paragraph{Highly Critical}\label{sec:deployment_standardization:standardization:highly_critical} To guarantee global connectivity, only one routing algorithm for this purpose must be standardized. Furthermore, the basic format of PCBs, which contains the necessary information to specify paths, must be standardized as mandatory fields.



\paragraph{Moderately Critical}\label{sec:deployment_standardization:standardization:moderately_critical} For path optimization on basic criteria, we recommend the standardization of one algorithm per basic criterion. To enable the communication of performance metrics associated with basic criteria, the static info extension (\Cref{sec:pan}) must be defined as optional PCB fields. To ensure extensibility, instead of standardization, the extension for different basic performance metrics must be published in one public append-only list with one format per metric. 
% Originally there was a comment here, but removed for overview;
% tabaeeali: Not sure if this is the right way to go.
% Mar 27, 2023 6:45 PM
% tabaeeali: should it be append-only?
% Mar 28, 2023 2:11 PM

\paragraph{Non-Critical}\label{sec:deployment_standardization:standardization:non_critical} Routing algorithms are not standardized, allowing each AS to freely choose any  algorithm it wants to deploy, and allowing end ASes to specify any on-demand algorithm they want to be communicated via PCBs. Since ASes need a common understanding of path performance metrics, the formats of static info extension for arbitrary metrics also needs to be published in a public list. In this tier, on-demand routing (\Cref{sec:principles:on_demand}) is the replacement for algorithm standardization as it ensures all ASes run the same algorithm which is communicated via PCBs without knowing any standards and deploying them in advance, ensuring optimality, real-time extensibility, and zero standardization efforts altogether.

\paragraph{Backward-Compatibility} Since deploying \system{} is optional, some ASes may still use SCION's legacy control plane. To guarantee connectivity among all SCION ASes, not just the ones deploying \system{}, the standardized connectivity algorithm and basic PCB format must be backward-compatible with the legacy control plane.


\paragraph{\system{}-Specific Efforts}\label{sec:deployment_standardization:standardization:non_critical} To allow effortless deployment of new algorithms and to enable on-demand routing, the interface between RAC (\Cref{sec:internal_architecture:rac}) and the algorithm must be standardized. With a standardized interface, every algorithm can be deployed in any AS, facilitating the proposal of new open-source algorithms that ASes can deploy effortlessly, enhancing extensibility. Furthermore, to enable on-demand routing (\Cref{sec:principles:on_demand}), pull-based routing (\Cref{sec:principles:pull_based}), and flexible optimization granularity (\Cref{sec:principles:granularity}), their corresponding PCB extensions (\Cref{sec:principles:pcb_extensions}) must be standardized as optional PCB fields.
  
\subsection{Deployment Requirements}\label{sec:deployment_standardization:deployment:highly_critical}
The general deployment requirement is the prioritization of more critical tiers over less critical ones. Within each tier, we propose the following requirements:

\paragraph{Highly Critical}\label{sec:deployment_standardization:deployment:highly_critical} All ASes must deploy the only standardized algorithm of this tier, which is designed for connectivity. Otherwise, connectivity is not guaranteed.

\paragraph{Moderately Critical}\label{sec:deployment_standardization:deployment:moderately_critical} ASes can choose whether they want to participate in path optimization for basic criteria, and if so, which criteria and with which algorithm. However, to improve path quality, we recommend ASes the deployment of all standardized algorithms of this tier and prioritizing them over non-standardized algorithms. 

\paragraph{Non-Critical}\label{sec:deployment_standardization:deployment:non_critical} Although ASes are free to deploy any algorithms, we recommend to prioritize support for on-demand algorithms over locally selected algorithms to ensure optimality without need for standardization (\Cref{sec:deployment_standardization:standardization:non_critical}).
